On the Benefits of Large Learning Rates for Kernel Methods

This paper studies an intriguing phenomenon related to the good generalization performance of estimators obtained by using large learning rates within gradient descent algorithms. First observed in the deep learning literature, we show that a phenomenon can be precisely characterized in the context of kernel methods, even though the resulting optimization problem is convex. Specifically, we consider the minimization of a quadratic objective in a separable Hilbert space, and show that with early stopping, the choice of learning rate influences the spectral decomposition of the obtained solution on the Hessian's eigenvectors. This extends an intuition described by Nakkiran (2020) on a two-dimensional toy problem to realistic learning scenarios such as kernel ridge regression. While large learning rates may be proven beneficial as soon as there is a mismatch between the train and test objectives, we further explain why it already occurs in classification tasks without assuming any particular mismatch between train and test data distributions.

==> sections/2d_case.tex <==

Consider the following simplified settings. We have $\HH = \RR^2$, $\optEmp = \optPop = 0$, $\TEmp = \Diag \p{\sigma_1, \sigma_2}$, and $\TPop = \II_2$. With $(e_1, e_2)$ the canonical basis of $\RR^2$ (which is also the eigenbasis of $\TEmp$), we assume $\theta_0 = (\iota, \iota)$, for $\iota \in \RR$. Then, we denote the estimator at step $t$ with $\theta_{\eta, t} = (x_{(t, \eta)}, y_{(t, \eta)})$. Simple calculus then shows that
\begin{equation}\label{eq:sketch_proof_notations}
    \LEmp(\theta_{\eta, t}) = \frac{1}{2} \sigma_1 x_{(t, \eta)}^2 + \frac{1}{2} \sigma_2 y_{(t, \eta)}^2, ~~ \andtext ~~ \p{\begin{matrix} x_{(t, \eta)} \\ y_{(t, \eta)} \end{matrix}}
    = \p{\begin{matrix} (1 - \eta \sigma_1)^t \iota \\  (1 - \eta \sigma_2)^t \iota \end{matrix}}.
\end{equation}

\paragraph{Small learning rate.} 
Consider the estimator $\theta_s$ obtained with $t_s$ steps with learning rate $\eta_s < 2 / (\sigma_1 + \sigma_n)$. We drop the $\eta, t$ upperscript in this paragraph. Then, we have that $(1 - \eta_s \sigma_1) < (1 - \eta \sigma_2)$ (refer to \cref{fig:attenuation_coefficient_function_lr} for a visual). Thus, the quantity:
\begin{equation*}
    \epsilon_s^2 = \frac{x_s^2}{y_s^2} = \p{\frac{1 - \eta_s \sigma_1}{1 - \eta_s \sigma_2}}^{2 t_s}
\end{equation*}
goes to $0$ when $t_s \to \infty$. Specifically, we have that
\begin{equation}\label{eq:sketch_small_bound_eps}
    t \geq t_{s, 1} \eqdef \frac{1}{2}\frac{ \log2 \sigma_1 / \sigma_2}{\log \frac{1 - \eta_s \sigma_1}{1 - \eta_s \sigma_2}} \implies \epsilon_s^2 \leq \frac{\sigma_2}{2 \sigma_1}.
\end{equation}
On the other hand, we can bound the empirical loss in two ways. With the definition of $\LEmp$ in \cref{eq:sketch_proof_notations} we have that
\begin{equation*}
    \sigma_2 y_s^2 \leq \LEmp(\theta_s) = \sigma_2 y_s^2 (1 + \epsilon_s^2 \sigma_1/\sigma_2)/2~~ \andtext ~~ \alpha/2 \leq \LEmp(\theta_s) \leq \alpha.
\end{equation*}
where the second inequality holds by assuming that $\theta_s$ belongs to the $(\alpha/2, \alpha)$ level-sets of $\LEmp$.

On the other hand, we want $\theta_s$ to belong to the $\alpha/2, \alpha$ level set of $\LEmp$. Assuming $t \geq t_{s, 1}$, we aim for
\begin{equation}
    \frac{\alpha}{2} < \frac{1}{2} \sigma_2 \mu_{s, 2}^2 < \LEmp(\theta_s) = \frac{1}{2} (\sigma_1 \mu_{s, 1}^2 + \sigma_2 \mu_{s, 2}^2) < \frac{1}{2} \sigma_2 \mu_{s, 2}^2 (1 + \frac{\sigma_1}{\sigma_2}\epsilon_s^2) < \alpha.
\end{equation}
This can be rewritten 
\begin{equation}\label{eq:sketch_small_lr_1}
    \frac{1}{2} \alpha \leq \frac{1}{2} \sigma_2 \mu_{s,2}^2 \leq \frac{2}{3} \alpha,
\end{equation}
as we assumed $t \geq t_{s, 1}$ which allows to bound $\epsilon_s^2$ using \cref{eq:sketch_small_bound_eps}. Using the closed-form expression of $\mu_{s, 2}$, we can express condition on $t_s$ for \cref{eq:sketch_small_lr_1} to be satisfied. Specifically, we have 
\begin{equation}
    \frac{1}{2} \frac{\log \frac{\alpha}{\sigma_2 \iota}}{\log 1 - \sigma_2 \eta_s} 
    \eqdef t_{s,2} < t < t_{s,3} \eqdef
    \frac{1}{2} \frac{\log \frac{4}{3} \frac{\alpha}{\sigma_2 \iota}}{\log 1 - \sigma_2 \eta_s} \implies \text{\cref{eq:sketch_small_lr_1} holds}.
\end{equation}
To conclude, we need to check that $t_{s,2} > t_{s, 1}$. Otherwise, we can't write \cref{eq:sketch_small_lr_1}. Looking at the definition of $t_{s, 1}$ and $t_{s,2}$, this is achieved by setting $\alpha / \iota$ sufficiently small.\todo{Small $\eta_s$ works fine too.} 

Thus, $\theta_s$ is in the $(\alpha/2, \alpha)$ level sets of $\LEmp$ and satisfies 
\begin{equation}\label{eq:sketch_small_lr_final}
    \LPop(\theta_s) = \mu_{s, 1}^2 + \mu_{s, 2}^2 \geq \mu_{s, 2}^2 \geq \frac{\alpha}{\sigma_2}.
\end{equation}

\paragraph{Big learning rate.}
We proceed in a similar way with $\theta_b$, the estimator obtained with $t_b$ steps with learning rate $\eta_b > 2 / (\sigma_1 + \sigma_2)$. Then, notice that $|1 - \eta_b \sigma_1| > 1 - \eta_n \sigma_2$, so, by a similar reasoning, we have that 
\begin{equation}
    t \geq t_{b, 1} \eqdef \frac{1}{2}\frac{ \log 1/2}{\log \frac{\absv{1 - \eta_b \sigma_1}}{1 - \eta_b \sigma_2}} \implies \epsilon_b^2 \eqdef \frac{\mu_{b, 2}^2}{\mu_{b, 1}^2}\leq 1/2.
\end{equation}
Again, the bound on $\LEmp(\theta_b)$ can be derived with 
\begin{equation}
    \frac{\alpha}{2} < \frac{1}{2} \sigma_1 \mu_{b, 1}^2 < \LEmp(\theta_s) = \frac{1}{2} (\sigma_1 \mu_{b, 1}^2 + \sigma_2 \mu_{b, 2}^2) < \frac{1}{2} \sigma_1 \mu_{b, 1}^2 (1 + \epsilon_b^2) < \alpha
\end{equation}
and it $t \geq t_{b, 1}$, then $\epsilon_{1, b}^2 \leq 1/2$ so that
\begin{equation}
    \frac{1}{2} \frac{\log \frac{\alpha}{\sigma_1 \iota}}{\log 1 - \sigma_1 \eta_b} 
    \eqdef t_{b,2} < t < t_{b,3} \eqdef
    \frac{1}{2} \frac{\log \frac{4}{3} \frac{\alpha}{\sigma_1 \iota}}{\log 1 - \sigma_1 \eta_b} \implies \frac{1}{2} \alpha \leq \frac{1}{2} \sigma_1 \mu_{b, 1}^2 \leq \frac{2}{3} \alpha.
\end{equation}
With the same remark on the ratio $\iota / \alpha$ to be sufficiently big so that $t_2 > t_1$, we can give an upper bound on the risk of $\theta_b$, with
\begin{equation}\label{eq:sketch_big_lr_final}
    \LPop(\theta_b) = \mu_{b, 1}^2 + \mu_{b, 2}^2 \leq \mu_{b, 1}^2 (1 + \epsilon_b^2) \leq \frac{2}{3} \mu_{b, 1}^2 \leq \frac{8}{9} \frac{\alpha}{\sigma_1}.
\end{equation}

\paragraph{Conclusion.}
By combining \cref{eq:sketch_small_lr_final,eq:sketch_big_lr_final}, we obtain
\begin{equation}
    \frac{\LPop(\theta_s)}{\LPop(\theta_b)} \geq \frac{9}{8} \frac{\sigma_1}{\sigma_2}.
\end{equation}


==> sections/computational_complexity.tex <==
Consider the range of number of steps given in \cref{eq:prop_numerical_bound_nb_steps_small,eq:prop_numerical_bound_nb_steps_big}. In practical settings, one would stop the gradient descent as soon as the training loss is smaller than $\alpha$. Thus, we focus on the lower bound (we highlighted that the upper bound is not relevant in practice when we introduced Lemma~\ref{lem:upper_bound_steps}) and define 
\begin{align*}
    t_s &= \frac{1}{\hlmathblue{\log \frac{A_{s, n}}{\bar{A}_{s}}}} \max \cb{ \frac{1}{2} \log \frac{4 \hlmathgreen{\zeta_s^2}}{\tau}, \log 8 \kappa_{\tilde{T}} \hlmathgreen{\xi_s}}, \\
    t_b &= \frac{1}{\hlmathblue{\log \frac{A_{b, 1}}{\bar{A}_{b}}}} \max \cb{ \frac{1}{2} \log \frac{4 \hlmathgreen{\zeta_b^2}}{\tau}, \log 2 \kappa_{\tilde{T}} \hlmathgreen{\xi_b}}.
\end{align*}

The terms $\zeta_s, \zeta_b, \xi_s$ and $\xi_b$ depend on the initialization, and their analysis is not straigthforward\todo{Write it!}. On the other hand, the quotient in $A_x$ depend on the step size $\eta$. We consider 3 situations: small step size with $\eta \ll 1/\sigma_1$, optimal step size with $\eta = 1/\sigma_1$, and large step size with $\eta = 2/\sigma_1$. 

\subsection{Experimental study}

We look at the number of steps to achieve $0.05$ training loss on $n=1000$ samples of CKN-MNIST without regularization depending on the variance at initialization $\alpha_0 = \mathcal{U}(-\tau, \tau)$ and the learning rate. We look at $\eta \in \csb{.99 \frac{2}{\sigma_1}, \frac{1}{\sigma_1}, \frac{1}{2\sigma_1}}$.\gaspard{Use $.99$ to learn slowly the first component. Otherwise need annealing strategy, annoying.}

\begin{figure}
    \centering
    \includegraphics[width=.3\linewidth]{figures/complexity/train/complexity_gd_tau10.png}
    \hfill
    \includegraphics[width=.3\linewidth]{figures/complexity/train/complexity_gd_tau1.png}
    \hfill
    \includegraphics[width=.3\linewidth]{figures/complexity/train/complexity_gd_tau0.001.png}

    \includegraphics[width=.3\linewidth]{figures/complexity/hilbert/complexity_gd_tau10.png}
    \hfill
    \includegraphics[width=.3\linewidth]{figures/complexity/hilbert/complexity_gd_tau1.png}
    \hfill
    \includegraphics[width=.3\linewidth]{figures/complexity/hilbert/complexity_gd_tau0.001.png}

    \caption{Number of steps function of the step size, when doing gradient descent on the train loss \textit{(top)} or on the Hilbert norm \textit{(bottom)}. It depends on the variance, \textit{(left)} big variance, \textit{(center)} medium, and \textit{(right)} close to 0. Error bars are standard deviation over 5 runs.}
\end{figure}

\subsection{Terms depending on the initialization}

We have that 
\begin{equation*}
    \iota_i \eqdef \dotprod{\theta_{0} - \optEmp}{e_i}_\HH = \sqrt{n\sigma_i} \dotprod{\alpha_0 - \alpha^\star}{u_i}_{\RR^n},
\end{equation*}
where $(\sigma_i, u_i)$ are eigenpairs of $K/n$. We distinguish between two cases: \textit{(i)} initialization with high variance, where $\alpha_0 \gg \alpha^\star$, and \textit{(ii)} initialization close to 0. 

\paragraph{Large variance initialization.}
In this case,
\begin{equation*}
    \iota_i \approx \sqrt{n \sigma_i} \alpha_0^\top e_i,
\end{equation*}
and if $\alpha_0$ is sampled uniformly on the sphere, then so is $U^\top \alpha_0$. 

\paragraph{Low variance initialization.}
Then 
\begin{equation*}
    \iota_i \approx \sqrt{n \sigma_i} {\alpha^\star}^\top e_i.
\end{equation*}
We can define $\alpha^\star$ with a spectral filter $g_\lambda$, with
\begin{equation*}
    \alpha^\star = \frac{1}{n} g_\lambda\p{\frac{K}{n}} y.
\end{equation*}
Thus, if we regularize, $\iota_i$ will be bigger on the low-frequency component. 


\subsection{Attenuation coefficients}

\paragraph{Small step size.}
We set $\eta \leq 1/\sigma_1$. Then, following the discussion of \cref{eq:def_admissible_lr_small_big}, the attenuation coefficient satisfy 
\begin{equation*}
    \forall i < n-1, ~~ 1 - \eta \sigma_n = A_n > A_{n-1} = 1 - \eta \sigma_{n-1} > A_i.
\end{equation*}
We obtain 
\begin{equation}\label{eq:log_ratio_attenuation_small_lr}
    \log \frac{A_{s, n}}{\bar{A}_{s}} = \log \frac{1 - \eta \sigma_{n}}{1 - \eta \sigma_{n-1}}.
\end{equation}
In the small step size limit, with $\eta = o(1)$, \cref{eq:log_ratio_attenuation_small_lr} becomes 
\begin{equation}
    \log \frac{A_{s, n}}{\bar{A}_{s}} = (\sigma_{n-1} - \sigma_n) \eta + o(\eta).
\end{equation}

\paragraph{Optimal step size.}
We set $\eta = 1/\sigma_1$. \cref{eq:log_ratio_attenuation_small_lr} becomes 
\begin{equation*}
    \log \frac{A_{s, n}}{\bar{A}_{s}} = \log \frac{1 - \sigma_{n}/\sigma_1}{1 - \sigma_{n-1}/\sigma_1}.
\end{equation*}
If we assume $\kappa_{\hat{T}} \gg 1$, we have 
\begin{equation}
    \log \frac{A_{s, n}}{\bar{A}_{s}} = \frac{\sigma_{n-1} - \sigma_n}{\sigma_1} + o(\kappa_{\hat{T}}^{-1}).
\end{equation}

\paragraph{Big step size.}
We set $\eta = 2/\sigma_1$. We consider the case where $A_n > A_2$, which occurs empirically as soon as we do not regularize. Following \cref{eq:def_admissible_lr_small_big}, we have
\begin{equation*}
    \log \frac{A_{b, 1}}{\bar{A}_{b}} = \log \frac{1}{1 - 2 \sigma_n / \sigma_1}.
\end{equation*}
Again, if we assume that $\kappa_{\hat{T}} \gg 1$, we have 
\begin{equation}
    \log \frac{A_{b, 1}}{\bar{A}_{b}} = \frac{2}{\kappa_{\hat{T}}} + o(\kappa_{\hat{T}}^{-1}).
\end{equation}



==> sections/filter_bound.tex <==
\begin{assumption}[Settings.]
    We assume
    \begin{equation}
        \exists c_m, c_M, \beta, ~~ c_m \TEmp^\beta \leq \TPop \leq c_M \TEmp^\beta
    \end{equation}
    This always hold at least with $c_m = \varsigma_n, c_M = \varsigma_1$ and $\beta=0$ which simply means that $\TPop$ is p.d. 
\end{assumption}

\subsection{Expressing the filter}

We have the following inequalities:
\begin{align*}
    \LPop(\theta_b) 
    &= \frac{1}{2} \norm{\theta_b - \optPop}_\TPop^2 \\
    &\leq \norm{\theta_b - \optEmp}_\TPop^2 + \norm{\optEmp - \optPop}_\TPop^2 \\
    &= \norm{(\II - \eta_b \TEmp)^{t_b} (\theta_0 - \optEmp)}_\TPop^2 + 2 \LPop(\optEmp) \\ 
    &= \norm{\TPop^{1/2}(\II - \eta_b \TEmp)^{t_b} (\II - \eta_s \TEmp)^{-t_s} \TPop^{-1/2} \TPop^{1/2} (\II - \eta_s \TEmp)^{t_s} (\theta_0 - \optEmp)}_\HH^2 + 2 \LPop(\optEmp) \\ 
    &\leq \norm{\TPop^{1/2}(\II - \eta_b \TEmp)^{t_b} (\II - \eta_s \TEmp)^{-t_s} \TPop^{-1/2}}^2 \norm{\theta_s - \optEmp}_\TPop^2 + 2 \LPop(\optPop)
\end{align*}
We bound $\norm{\theta_s - \optEmp}_\TPop^2$ with 
\begin{equation*}
    \norm{\theta_s - \optEmp}_\TPop^2 \leq 2 (\norm{\theta_s - \optPop}_\TPop^2 + \norm{\optEmp - \optPop}_\TPop^2) = 4 (\LPop(\theta_s) + \LPop(\optEmp))
\end{equation*}
and by defining 
\begin{equation}
    A = \norm{\TPop^{1/2}(\II - \eta_b \TEmp)^{t_b} (\II - \eta_s \TEmp)^{-t_s} \TPop^{-1/2}}^2
\end{equation}
we have 
\begin{equation}
    \LPop(\theta_b) 
    \leq 4 A \LPop(\optEmp_s) + 4 (1 + A) \LPop(\optEmp)
\end{equation}
If $A \to 0$, we deduce that big step size are better than small step size up to the model error $\LPop(\optEmp)$. Otherwise, we can't say anything. 

We now proceed to bounding $A$.

\subsection{Bounding the filter}

With the assumption on $\TPop$, we have 
\begin{equation}
    A = \sqrt{\frac{c_M}{c_m}} \cdot \max_{1 \leq i \leq n} \cb{ 
        h(\sigma_i) 
        \eqdef \absv{\frac{(1 - \eta_b \sigma_i)^{t_b}}{(1 - \eta_s \sigma_i)^{t_s}}}
    }
\end{equation}
Note that 
\begin{equation*}
    (\log h(\sigma))' = - \frac{\eta_b t_b}{1 - \eta_b \sigma} + \frac{\eta_s t_s}{1 - \eta_s \sigma}.
\end{equation*}
\todo{Ongoing work below. We can have bounds involving the training loss without too much issue I think.}

\begin{assumption}[Step size and number of steps.]\label{asmpt:subcases_filter}
    We assume:
    \begin{equation}
        \eta_s < \frac{1}{\sigma_1} < \eta_b < \frac{2}{\sigma_1}
    \end{equation}
    and 
    \begin{equation}
        t_b \geq t_s
    \end{equation}
    The other cases are easy to deal with, just need to write them down. But this one is the most interesting and straightforward.
\end{assumption}

\subsection{Technical result}

In fact, all the result boils down to the following lemma.

Define
\begin{equation}
    h(\sigma) = \frac{\absv{1 - \eta_b \sigma}^{t_b}}{\absv{1 - \eta_s \sigma}^{t_s}} \sigma^\beta, ~~ \beta \in \cb{-1/2, 0, 1/2}.
\end{equation}
We are interested in 
\begin{equation*}
    A = \sup_{1 \leq i \leq n} h(\sigma_i),
\end{equation*} 
for which we introduce the derivative of the logarithm to study its variation
\begin{equation}
    l(\sigma) = \frac{\beta}{\sigma} - \frac{\eta_b t_b}{1 - \eta_b \sigma} + \frac{\eta_s t_s}{1 - \eta_s \sigma}.
\end{equation}

\paragraph{Case $\beta=0$.}
Then 
\begin{equation}\label{eq:beta_0_derivative}
    l(\sigma) = \frac{1}{(1 - \eta_b \sigma) (1 - \eta_s \sigma)} \cdot \p{(\eta_s t_s - \eta_b t_b) + \eta_s \eta_b (t_b - t_s) \sigma}.
\end{equation}

We look at $(\eta_s t_s - \eta_b t_b) + \eta_s \eta_b (t_b - t_s) \sigma$. It is negative as long as 
\begin{equation*}
    \sigma < \frac{t_b/\eta_s - t_s / \eta_b}{t_b - t_s} \eqdef s_1,
\end{equation*}
positive otherwise. However, notice that
\begin{align*}
    \sigma_1 < s_1 \iff \eta_s < \frac{t_b \eta_b}{\sigma_1 \eta_b(t_b - t_s) + t_s} \eqdef \eta_1
\end{align*}
As a function of $t_b$, \emph{i.e.} $t_b \mapsto \eta_1(t_b)$, we have that $\eta_1$ is a decreasing function of $t_b$, with $\eta_1(t_s) = \eta_b$ and $\lim_{t_b \to \infty} \eta_1 = 1/\sigma_1$. Thus,
\begin{equation*}
    \forall t_b, ~~ \eta_1 > 1/\sigma_1, ~~ \text{which implies that} ~~ \sigma_1 < s_1.
\end{equation*}
Thus, $(\eta_s t_s - \eta_b t_b) + \eta_s \eta_b (t_b - t_s) \sigma$ is negative on $\csb{\sigma_n, \sigma_1}$.

Back to \cref{eq:beta_0_derivative}, we see that $l$ is negative on $[\sigma_n, 1/\eta_b]$ and positive in $[1/\eta_b, \sigma_1]$. So $h$ has its maximum in $\sigma_n$. This gives 
\begin{equation}
    A = \frac{(1 - \eta_b \sigma_n)^{t_b}}{(1 - \eta_s \sigma_n)^{t_s}} \to 0 ~~ \text{when} ~~ t_b \geq t_s \to \infty.
\end{equation}

\paragraph{Case $\beta=-1/2$.}
Then 
\begin{equation*}
    l(\sigma) = - \frac{1}{2\sigma} - \frac{\eta_b t_b}{1 - \eta_b \sigma} + \frac{\eta_s t_s}{1 - \eta_s \sigma}.
\end{equation*}
Remark that by multiplying $l$ by $2\sigma (1 - \eta_b \sigma) (1 - \eta_s \sigma)$, we can consider the polynom
\begin{equation*}
    P_1(\sigma) = \sigma^2 \eta_b \eta_s (-1 + 2(t_b - t_s)) + \sigma((\eta_b + \eta_s) - 2(\eta_b t_b - \eta_s t_s)) - 1.
\end{equation*}
As $(1 - \eta_b \sigma) > 0$ when $\sigma < 1/\eta_b$, then $l$ has the same sign to $P_1$ on $[0, 1/\eta_b]$. On the otherhand, it has the opposite sign on $[1/\eta_b, \sigma_1]$. Now, denote $s_1$ the second root of $P_1$, which is a positive parabola as soon as $t_b \geq t_s + 1$. we have that 
\begin{equation}
    \forall \sigma \leq 1/\eta_b, ~~ l(\sigma) < 0 ~~ \iftext ~~ \sigma < s_1.
\end{equation}


==> sections/old_proof.tex <==
\subsection{First step: a bound on the population losses}

We start by using the definition of the population loss, that is 
\begin{equation*}
    L(\theta) = \frac{1}{2} \norm{\theta - \optPop}_{\TPop^\beta}^2,
\end{equation*}

\paragraph{Upper bound for big learning rate.}
We use the decomposition
\begin{equation*}
    \theta_{b} - \optPop = \theta_{b} - \optEmp + \optEmp - \optPop = \sum_{i=1}^n {\mu_{b,i}} e_i + \optEmp - \optPop,
\end{equation*}
to obtain, by triangular inequality and $(a+b+c)^2 \leq 3 (a^2 + b^2 + c^2)$, 
\begin{equation*}
    L(\theta_{b}) \leq 3 \p{\frac{1}{2}\mu_{b,1}^2\norm{e_1}_{\TPop^\beta}^2 + \frac{1}{2} \norm{\optEmp - \optPop}_{\TPop^\beta}^2 + \frac{1}{2} \norm{ \sum_{i=2}^n \mu_{b,i} e_i}_{\TPop^\beta}^2}.
\end{equation*}
We define
\begin{equation}\label{eq:def_eps_st_eps_2b_eps_3b}
    \epsilon_{ST}^2 = \frac{1}{2}\norm{\optEmp - \optPop}_{\TPop^\beta}^2, ~~ \epsilon_{2,b}^2 = \frac{\epsilon_{ST}^2}{\nicefrac12 \norm{\mu_{b,1}e_1}_{\TPop^\beta}^2} ~~ \andtext ~~ \epsilon_{3, b}^2 = \frac{\norm{ \sum_{i=2}^n \mu_{b,i} e_i}_{\TPop^\beta}^2}{\norm{\mu_{b,1}e_1}_{\TPop^\beta}^2}.
\end{equation}
$\epsilon_{ST}$ is the statistical error; $\epsilon_{2,b}$ is the statistical error normalized by a quantity depending on $\theta_{b}$; and $\epsilon_{3,b}$ is the relative population error when approximating $\theta_{b}$ by the projection on the first eigenvector. With these notations, we obtain
\begin{equation}\label{eq:pop_loss_lower_bound}
    L(\theta_{b}) \leq \frac{3}{2} \norm{\mu_{b,1}e_1}_{\TPop^\beta}^2 \p{1 + \epsilon_{2,b}^2 + \epsilon_{3,b}^2}.
\end{equation}

\paragraph{Lower bound for small learning rate.}
Similarly to the big learning rate, we use the decomposition
\begin{equation*}
    \theta_{s} - \optPop = \theta_{s} - \optEmp + \optEmp - \optPop = \sum_{i=1}^n \mu_{i, s} e_i + \optEmp - \optPop.
\end{equation*}
We have:
\begin{equation*}
        L(\theta_{s}) \geq \frac{1}{2} \p{ \norm{\mu_{s,n} e_n}_{\TPop^\beta} - \norm{\sum_{i<n} \mu_{s,i} e_i}_{\TPop^\beta} - \norm{\optEmp - \optPop}_{\TPop^\beta}}^2
\end{equation*}
next observe that $(a-b-c)^2 = a^2 (1 - (b+c)/a)^2 \geq a^2 (1 - 2 (b+c)/a)$. Plugging this in the r.h.s of the previous equation, we obtain
\begin{equation}\label{eq:pop_loss_upper_bound}
    L(\theta_{s}) \geq \frac{1}{2} \norm{\mu_{s,n} e_n}_{\TPop^\beta}^2 \p{1 - 2 (\epsilon_{2,s} + \epsilon_{3,s})},
\end{equation}
where we introduced, similarly to \cref{eq:def_eps_st_eps_2b_eps_3b},
\begin{equation}\label{eq:def_eps_2s_3s}
    \epsilon_{2,s}^2 = \frac{ 2 \epsilon_{ST}^2}{\norm{\mu_{s,n} e_n}_{\TPop^\beta}^2} ~~ \andtext ~~ \epsilon_{3,s} = \frac{\norm{\sum_{i<n}\mu_{s,i} e_i}_{\TPop^\beta}}{\norm{\mu_{s,n} e_n}_{\TPop^\beta}}.
\end{equation}

\paragraph{Combining the two bounds.}
We combine the lower bound on the population loss in \cref{eq:pop_loss_lower_bound} and the upper bound  of \cref{eq:pop_loss_upper_bound} to obtain 
\begin{equation}\label{eq:step_1_bound_population_loss}
    \frac{L(\theta_{s})}{L(\theta_{b})} \geq \frac{1}{3} \frac{\norm{\mu_{s,n} e_n}_{\TPop^\beta}^2 \p{1 - 2 (\epsilon_{2,s} + \epsilon_{3,s})}}{\norm{\mu_{b,1}e_1}_{\TPop^\beta}^2 \p{1 + \epsilon_{2,b}^2 + \epsilon_{3,b}^2}}.
\end{equation}

\subsection{Second step: a bound on the empirical losses}

The goal of this section is to bound $\mu_{s,n}/\mu_{b,1}$.

Recall that $\theta_{b}$ and $\theta_{s}$ both belong to the $\alpha$-level sets of the empirical loss $\LEmp$. Thus, we have that
\begin{equation*}
    \tau \alpha \leq \hat{L}(\theta_{s \text{ or } b}) = \frac{1}{2}\norm{\theta_{s \text{ or } b} - \optEmp}_{\hat{T}}^2 \leq \alpha.
\end{equation*}
Recalling that $\sigma_i$ is the $i$-th eigenvalue of $\TEmp$, we rewrite the empirical loss with 
\begin{equation*}
    \begin{aligned}
        \hat{L}(\theta_{b}) = \frac{1}{2} \sum_{i=1}^n \sigma_i \mu_{b,i}^2, \\
        \hat{L}(\theta_{s}) = \frac{1}{2} \sum_{i=1}^n \sigma_i \mu_{s,i}^2.
    \end{aligned}
\end{equation*}

Gradient descent with small step size will project the initial estimator towards the smallest eigenvector; next assumption ensures that such projection is not in the level-set $\alpha$ of the training loss. It is enforced as soon as the early stopping criterium is small enough.\todo{Check that it is used somewhere. It must.}
\begin{assumption}{Initial projection}\label{asmpt:initial_projection}
    We assume that 
    \begin{align}
        \alpha &\leq \frac{1}{2}\sum_{i<n} \sigma_i \iota_{i}^2 \label{eq:asmpt_initial_small_lr}\\
        \alpha &\leq \frac{1}{2}\sum_{i>1} \sigma_i \iota_{i}^2 \label{eq:asmpt_initial_big_lr}.
    \end{align}
    \cref{eq:asmpt_initial_small_lr} ensures that the projection on the first $n-1$ eigenvectors of $\theta_{0} - \optEmp$ is not in the level sets $\alpha$. \cref{eq:asmpt_initial_big_lr} ensures the same on the last $n-1$ eigenvectors. This is satisfied as soon as the objective training loss is small enough. Said differently, we require the random initialization to be bad enough so that optimization is required, which is fairly natural in practice. 
\end{assumption}

The first relation is easy: we simply write 
\begin{equation}\label{eq:upper_bound_mu_b1}
    \mu_{b, 1}^2 \leq \frac{1}{\sigma_1}\p{2\alpha - \sum_{i=2}^n \sigma_i \mu_{i, b}^2} \leq \frac{2\alpha}{\sigma_1}.
\end{equation}
Second relation is 
\begin{equation}\label{eq:lower_bound_mu_sn}
    \mu_{s, n}^2 \geq \frac{2 \tau \alpha}{\sigma_n}\p{1 - \epsilon_{4,s}^2},
\end{equation}
where we introduced 
\begin{equation}\label{eq:def_eps_4s}
    \epsilon_{4,s}^2 = \frac{\nicefrac{1}{2}\sum_{i<n} \sigma_i \mu_{s, i}^2}{\tau \alpha}.
\end{equation}
Thus, by combining \cref{eq:upper_bound_mu_b1,eq:lower_bound_mu_sn}
\begin{equation}\label{eq:step_2_bound_empirical_losses}
    \frac{\mu_{s, n}^2}{\mu_{b, 1}^2} \geq \kappa_{\hat{T}} \cdot\p{1 - \epsilon_{4,s}^2}.
\end{equation}

\subsection{Third step: combining all bounds}
Finally, we use 
\begin{equation*}
    \frac{\norm{e_n}_{\TPop^\beta}^2}{\norm{e_1}_{\TPop^\beta}^2} \geq \frac{1}{\kappa_{\TPopProj}^\beta},
\end{equation*}
as $e_1$ and $e_n$ are both unit-length vectors of $\HH$, and we inject the inequality into \cref{eq:step_1_bound_population_loss}, along with \cref{eq:step_2_bound_empirical_losses}, to obtain 
\begin{equation}
    \frac{L(\theta_{s})}{L(\theta_{b})} \geq \frac{\kappa_{\hat{T}}}{\kappa_{\TPopProj}^\beta} \times \frac{1}{3} (1 - \epsilon_{4,s}^2) \frac{\p{1 - 2 (\epsilon_{2,s} + \epsilon_{3,s})}}{\p{1 + \epsilon_{2,b}^2 + \epsilon_{3,b}^2}}
\end{equation}
All that remains is to bound the error terms. This is the purpose of next section. 

\subsection{Fourth step: bounding the error terms}\label{sec:bounding_error_terms}

\paragraph{Useful quantities.}
We first introduce the following quantities. 
\begin{definition}[Quantities which depend on the initialization]\label{def:quantities_initialization}
    We define the following quantities, which depend on the initialization. 
    \begin{align}
        \iota_{\max} &= \max_{1 \leq i \leq n} \iota_i \\
        \zeta_s^2 &= \sum_{i<n} \frac{\sigma_i \iota_{i}^2}{\sigma_n \iota_n^2} \leq \frac{\iota_{\max}}{\iota_n} \frac{\norm{\hat{T}}_{\infty}}{\sigma_n} \leq n \frac{\iota_{\max}}{\iota_n} \kappa_{\hat{T}} \label{eq:def_zeta}\\
        \zeta_b^2 &= \sum_{i>1} \frac{\sigma_i \iota_{i}^2}{\sigma_1 \iota_1^2} \\
        \xi_s &= \sum_{i < n} \absv{\frac{\iota_i}{\iota_n}} \label{eq:def_xi_s}\\ 
        \xi_b &= \sum_{i > 1} \absv{\frac{\iota_i}{\iota_1}}
    \end{align}
\end{definition}
\begin{remark}[Interpretation of $\zeta_s$.]\label{rmk:interpretation_zeta_s}
    If we denote $P_n = e_n e_n^\top$ the projection on the $n$-th eigenspace, $\zeta_s$ can be rewritten
    \begin{equation*}
        \zeta_s^2 = \frac{\nicefrac{1}{2}\csb{P_n^\perp (\theta_{0} - \optEmp) ^\top} \TEmp \csb{P_n^\perp (\theta_{0} - \optEmp)} }{\nicefrac{1}{2}\csb{P_n (\theta_{0} - \optEmp) ^\top} \TEmp \csb{P_n (\theta_{0} - \optEmp)} }
    \end{equation*}
    which is the quotient of the training loss of the initialization projected on $P_n$ and $P_n^\perp$.
\end{remark}

Then, we have the second biggest amplification factors, depending on which step size we chose. 
\begin{definition}[Attenuation coefficients.]\label{def:attenuation_coeff}
    We introduce
    \begin{align}
        \bar{A}_s &= \max_{i < n} A_i \label{eq:def_barA_s} \\
        \bar{A}_b &= \max_{i > 1} A_i.
    \end{align}
    \textbf{Note that $\bar{A}_s$ and $\bar{A}_b$ both depends on the step size $\eta$}, which is constrained to $\eta_s < 2/(\sigma_1 + \sigma_n)$ and $\eta_b > 2/\sigma_1 - 2/(\sigma_1 + \sigma_n)$. 
\end{definition}

\paragraph{Empirical-based errors.}
Here we focus on $\epsilon_{4,s}$, to obtain
\begin{equation}
    1 - \epsilon_{4, s}^2 \geq 1/C ~~ \text{with} ~~ C > 1.
\end{equation}
We also need to introduce a similar quantity for $\theta_{b}$. We define, analogously to $\epsilon_{4,s}$ in \cref{eq:def_eps_4s}, 
\begin{equation}\label{eq:def_eps_4b}
    \epsilon_{4,b}^2 = \frac{\sum_{i>1} \sigma_i \mu_{b, i}^2}{2 \tau \alpha}.
\end{equation}
\begin{lemma}{Bounding $\epsilon_{4}$}\label{lem:bound_eps_4}
    Let $\delta > 0$. The following holds:
    \begin{align}
        t &\geq \frac{1}{2} \frac{\log \frac{\zeta_s^2}{\tau \delta^2}}{\log \frac{A_{s, n}}{\bar{A}_{s}}} \implies \epsilon_{4,s} \leq \delta, \\
        t &\geq \frac{1}{2} \frac{\log \frac{\zeta_b^2}{\tau \delta^2}}{\log \frac{A_{b, 1}}{\bar{A}_{b}}} \implies \epsilon_{4,b} \leq \delta.
    \end{align}
\end{lemma}

\begin{proof}
    We recall the definition of $\epsilon_{4,s}$ in \cref{eq:def_eps_4s}:
    \begin{equation*}
        \epsilon_{4,s}^2 = \frac{\sum_{i<n} \sigma_i \mu_{s, i}^2}{2 \tau \alpha}.
    \end{equation*}
    We can control this error as follows. Note that
    \begin{equation*}
        \alpha \geq \frac{1}{2}\p{\sigma_n \mu_{s,n}^2 + \sum_{i<n} \sigma_i \mu_{s,i}^2} \geq \tau \alpha ~~ \text{hence} ~~ 2 \alpha \geq \sigma_n \mu_{s,n}^2,
    \end{equation*}
    as $\theta_{s}$ belongs to the $\alpha$ level sets of $\LEmp$. Thus, the error can be written 
    \begin{equation*}
        \epsilon_{4, s}^2 = \frac{\sum_{i<n} \sigma_i \mu_{s, i}^2}{2 \tau \alpha} \leq \frac{1}{\tau} \frac{\sum_{i<n} \sigma_i \mu_{s, i}^2}{\sigma_n \mu_{s,n}^2} \eqdef M.
    \end{equation*}
    We now proceed to bounding $M$ by leveraging the fact that $\theta_{s}$ will be mostly directed along the smallest eigenvector of $\hat{T}$. By definition of $\mu_i$ in \cref{eq:def_iota_mu} and of $\zeta_s^2$ in \cref{eq:def_zeta}, we have 
    \begin{equation*}
        M = \frac{1}{\tau} \frac{\sum_{i<n} \sigma_i \iota_i^2 A_{s,i}^{2t}}{\sigma_n \iota_n^2 A_{s,n}^{2t}} \leq \frac{1}{\tau} \zeta_s^2 \p{\frac{\bar{A}_{s}}{A_{s, n}}}^{2t}.
    \end{equation*}
    Remember that by definition of the step size in \cref{eq:def_admissible_lr_small_big}, $\frac{\bar{A}_{s}}{A_{s, n}} \leq 1$.
    Thus, to have $\epsilon_{4, s}^2 \leq \delta^2$, it is sufficient to require
    \begin{equation*}
        \frac{1}{\tau} \zeta_s^2 \p{\frac{\bar{A}_{s}}{A_{s, n}}}^{2t} \leq \delta^2,
    \end{equation*}
    for which a sufficient condition is
    \begin{equation*}
        t \geq \frac{1}{2} \frac{\log \frac{\zeta_s^2}{\tau \delta^2}}{\log \frac{A_{s, n}}{\bar{A}_{s}}}.
    \end{equation*}
    We use the same reasoning for $\epsilon_{4, b}$, by splitting the sum on the first eigenvector rather than the last, \textit{i.e.} using
    \begin{equation*}
        \LEmp\p{\theta_{b}} = \sigma_1 \mu_{b, 1}^2 + \sum_{i>1}\sigma_i \mu_{b, i}^2.
    \end{equation*}
\end{proof}
\begin{remark}[Small learning rate limit]\label{rmk:eps4_small_learning_rate_limit}
    When $\eta \to 0$, we have $A_{s, n}/\bar{A}_s = (1 - \eta \sigma_n)/(1- \eta \sigma_{n-1})$ which gives 
    \begin{equation*}
        \frac{A_{s, n}}{\bar{A}_s} = 1 + (\sigma_{n-1} - \sigma_n)\eta + o(\eta), ~~\andtext ~~ \log \frac{A_n}{\bar{A}_s} = (\sigma_{n-1} - \sigma_n)\eta + o(\eta). 
    \end{equation*}
    Thus, in the small step size limit we have $t \sim 1/\eta$. 
\end{remark}

\paragraph{Population-based errors.}
In this paragraph, we bound $\epsilon_2$ and $\epsilon_3$. 

\begin{lemma}{Bounding $\epsilon_{2}$.}\label{lem:bound_eps_2}
    The following holds:
    \begin{align}
        \epsilon_{2,s} \leq \epsilon_{ST} \sqrt{\frac{\sigma_n / \tilde{\sigma}_n^\beta}{\tau\alpha (1 - \epsilon_{4,s}^2)}}, \\
        \epsilon_{2,b} \leq \epsilon_{ST} \sqrt{\frac{\sigma_1 / \tilde{\sigma}_n^\beta}{\tau\alpha (1 - \epsilon_{4,b}^2)}}.
    \end{align}
\end{lemma}
\begin{proof}
    The definition in \cref{eq:def_eps_2s_3s} is recalled here:
    \begin{equation}\label{eq:proof_bound_eps_2_eq1}
        \epsilon_{2,s} = \frac{ \sqrt{2}\epsilon_{ST}}{\norm{\mu_{s,n} e_n}_{\TPop^\beta}}.
    \end{equation}
    As $e_n$ is a unit-length vector, we have that $\norm{e_n}_{\TPop^\beta} \geq \tilde{\sigma}_n^{\beta/2}$, where $\tilde{\sigma}_n$ is the smallest eigenvalue of $\TPopProj$. Plugging into \cref{eq:proof_bound_eps_2_eq1}, we have
    \begin{equation}
        \epsilon_{2,s} \leq \epsilon_{ST} \frac{1}{\sqrt{\tilde{\sigma}_n^\beta}} \p{\frac{1}{2}\mu_{s,n}^2}^{-1/2}.
    \end{equation}
    Then, since $\theta_{s}$ is in the $\alpha$ level sets of $\LEmp$ we have, we can bound $\mu_{s, n}^2/2$ with \cref{eq:lower_bound_mu_sn} to obtain
    \begin{equation}
        \epsilon_{2,s} \leq \epsilon_{ST} \sqrt{\frac{\sigma_n}{\tilde{\sigma}_n^\beta} \cdot \frac{1}{\tau\alpha (1 - \epsilon_{4,s}^2)}} 
    \end{equation}

    The relation on $\epsilon_{2,b}$ follows the same reasoning, except that we use 
    \begin{equation*}
        \frac{1}{2}\mu_{b,1}^2 \geq \frac{\tau \alpha}{\sigma_1} (1 - \epsilon_{4, b}^2).
    \end{equation*}
\end{proof}

\begin{lemma}{Bounding $\epsilon_{3}$.}\label{lem:bound_eps_3}
    Let $\delta > 0$. The following holds:
    \begin{align}
        t &\geq \frac{\log \frac{\kappa_{\TPopProj}^\beta`' \xi_s}{\delta}}{\log \frac{A_{s,n}}{\bar{A}_s}} \implies \epsilon_{3,s} \leq \delta, \\
        t &\geq \frac{\log \frac{\kappa_{\TPopProj}^\beta`' \xi_b}{\delta}}{\log \frac{A_{b,1}}{\bar{A}_b}} \implies \epsilon_{3,b} \leq \delta.
    \end{align}
\end{lemma}
\begin{proof}
    The definition in \cref{eq:def_eps_2s_3s} is recalled here:
    \begin{equation}\label{eq:pop_based_1}
        \epsilon_{3,s} = \frac{\norm{\sum_{i<n}\mu_{s,i} e_i}_{\TPop^\beta}}{\norm{\mu_{s,n} e_n}_{\TPop^\beta}}.
    \end{equation}
    The $e_i$ are unit-length elements so $\norm{e_i}_{\TPop^\beta}/\norm{e_n}_{\TPop^\beta} \leq \kappa_{\TPopProj}^\beta$. Thus \cref{eq:pop_based_1} becomes
    \begin{equation}
    \epsilon_{3,s} \leq \frac{\sum_{i<n}\absv{\mu_{s,i}}}{\absv{\mu_{s,n}}} \kappa_{\TPopProj}^\beta.
    \end{equation}
    By definition of $(\mu_i)$ in \cref{eq:def_iota_mu}, we obtain 
    \begin{equation*}
        \epsilon_{3,s} \leq \frac{\sum_{i<n} \iota_i A_i^t}{\iota_n A_{s,n}^t} \kappa_{\TPopProj}.
    \end{equation*}
    \todo{Take square norm to make appear the norm at init.} Finally, using the definition of $\xi_s$ in \cref{eq:def_xi_s} and the one of $\bar{A}_s$ in \cref{eq:def_barA_s}, we have 
    \begin{equation*}
        \epsilon_{3,s} \leq \xi_s \p{\frac{\bar{A}_s}{A_{s,n}}}^t \kappa_{\TPopProj},
    \end{equation*}
    with $\bar{A}_s / A_{s,n} < 1$. Thus, for any $\delta > 0$, a sufficient condition for having $\epsilon_{3,s} \leq \delta$ is
    \begin{equation}
        \xi_s \p{\frac{\bar{A}_s}{A_{s,n}}}^t \kappa_{\TPopProj}^\beta \leq \delta \iff t \geq \frac{\log \frac{\kappa_{\TPopProj}^\beta \xi_s}{\delta}}{\log \frac{A_{s,n}}{\bar{A}_s}}.
    \end{equation}
    The same reasoning holds for $\epsilon_{3,b}$, with a big component on $e_1$ rather than $e_n$. 
\end{proof}

\paragraph{Preventing over-optimization.}
Our analysis rely on our final estimator being close to the $\alpha$-level set of the empirical loss, as stated in \cref{eq:estimator_in_level_set_alpha}. The lower bound is of purely theoretical help, to avoid an unnecessary complex analysis relying on learning rate annealing to reach \emph{exactly} $\alpha$ training error. Yet, we can provide upper bounds on the number of steps to avoid optimizing too much. There are quite loose. But again, we highlight they are not the aim of our paper. 

\begin{lemma}{Upper bound on the number of steps.}\label{lem:upper_bound_steps}
    Having 
    \begin{equation}
        \begin{cases}
            t_s \leq \frac{1}{2} \frac{\log \frac{\sigma_n \iota_n^2 }{2 \tau \alpha}}{\log \frac{1}{A_{s, n}}} \\
            t_b \leq \frac{1}{2} \frac{\log \frac{\sigma_1 \iota_1^2 }{2 \tau \alpha}}{\log \frac{1}{A_{b, 1}}}
        \end{cases}
    \end{equation}
    is sufficient to ensure 
    \begin{equation*}
        \hat{L}(\theta_{s}), \hat{L}(\theta_{b}) \geq \tau\alpha.
    \end{equation*}
\end{lemma}

\begin{proof}
    We simply use the following implication
    \begin{equation*}
        \frac{1}{2} \sigma_n \mu_{s, n}^2 \geq \tau\alpha \implies \hat{L}(\theta_{s}) = \frac{1}{2} \sum_{i=1}^n \sigma_i \mu_{s, i}^2 \geq \tau\alpha
    \end{equation*}
    and the result of the lemma follows from the definition of $\mu_{s, n}$ in \cref{eq:def_iota_mu}. 
\end{proof}

\paragraph{Numerical example.}
To fix ideas, the following proposition is a numerical example. 

\begin{proof}(Proof of \cref{prop:numerical_bound})
    To obtain this result, it is sufficient to enforce
    \begin{equation}
        \begin{cases}
            \epsilon_{4,s}^2 \leq 1/2, ~~ \epsilon_{4,b}^2 \leq 1/2 \\
            \epsilon_{2,s}, \epsilon_{3,s} \leq 1/8 \\
            \epsilon_{2,b}, \epsilon_{3,b} \leq 1/2
        \end{cases}
    \end{equation}
    in order to have
    \begin{equation*}
        \frac{1}{3} (1 - \epsilon_{4,s}^2) \frac{\p{1 - 2 (\epsilon_{2,s} + \epsilon_{3,s})}}{\p{1 + \epsilon_{2,b}^2 + \epsilon_{3,b}^2}} \geq \frac{1}{18}.
    \end{equation*}
    For the errors $\epsilon_{4,s}, \epsilon_{4,b}$, we use Lemma~\ref{lem:bound_eps_4} to require
    \begin{equation*}
        t_s \geq \frac{1}{2} \frac{\log \frac{4 \zeta_s^2}{\tau}}{\log \frac{A_{s, n}}{\bar{A}_{s}}},
        ~~ \andtext ~~ 
        t_b \geq \frac{1}{2} \frac{\log \frac{4 \zeta_b^2}{\tau}}{\log \frac{A_{b, 1}}{\bar{A}_{b}}}.
    \end{equation*}
    For the errors $\epsilon_{3,s}, \epsilon_{3, b}$, we use Lemma~\ref{lem:bound_eps_3} to enforce
    \begin{equation*}
        t_s \geq \frac{\log 8 \kappa_{\TPopProj} \xi_s}{\log \frac{A_{s,n}}{\bar{A}_s}}, 
        ~~ \andtext ~~ 
        t_b \geq \frac{\log 2\kappa_{\TPopProj} \xi_b}{\log \frac{A_{b,1}}{\bar{A}_b}}.
    \end{equation*}
    To sum up, we require of the number of steps to be 
    \begin{align}
        t_s &\geq \frac{1}{\log \frac{A_{s, n}}{\bar{A}_{s}}} \max \cb{ \frac{1}{2} \log \frac{4 \zeta_s^2}{\tau} , \log 8 \kappa_{\TPopProj} \xi_s}, \\
        t_b &\geq \frac{1}{\log \frac{A_{b, 1}}{\bar{A}_{b}}} \max \cb{ \frac{1}{2} \log \frac{4 \zeta_b^2}{\tau} , \log 2 \kappa_{\TPopProj} \xi_b}.
    \end{align}
    
    Finally, for the statistical errors $\epsilon_{2,s}, \epsilon_{2,b}$ we have Lemma~\ref{lem:bound_eps_2}. First, we use the fact that $\epsilon_{4,s}^2, \epsilon_{4,b}^2 \leq 1/2$ to have
    \begin{equation*}
        \epsilon_{2,s} \leq \epsilon_{ST} \sqrt{2 \frac{\sigma_n / \tilde{\sigma}_n}{\tau\alpha}},
        ~~ \andtext ~~
        \epsilon_{2,b} \leq \epsilon_{ST} \sqrt{2 \frac{\sigma_1 / \tilde{\sigma}_n}{\tau\alpha}}.
    \end{equation*}
    Thus, we require
    \begin{equation*}
        \frac{\epsilon_{ST}}{\sqrt{\tau\alpha}} \leq \frac{1}{8} \sqrt{\frac{1}{2} \frac{\tilde{\sigma}_n}{\sigma_n}},
        ~~ \andtext ~~
        \frac{\epsilon_{ST}}{\sqrt{\tau\alpha}} \leq \frac{1}{2} \sqrt{\frac{1}{2} \frac{\tilde{\sigma}_n}{\sigma_1}}.
    \end{equation*}
    As soon as $\hat{\kappa} \geq 16$, this simplifies to
    \begin{equation}
        \frac{\epsilon_{ST}^2}{\tau \alpha} \leq \frac{1}{8} \frac{\tilde{\sigma}_n}{\sigma_1}.
    \end{equation}    
\end{proof}

